Magnetic fields and plasma heating in the Sun's atmosphere

We use the first publically available data from the Daniel K. Inouye Solar Telescope (DKIST) to track magnetic connections from the solar photosphere into the corona. We scrutinize relationships between chromospheric magnetism and bright chromospheric, transition region and coronal plasmas. In June 2022, the Visible Spectro-Polarimeter (ViSP) instrument targeted unipolar network within a decaying active region. ViSP acquired rastered scans with longitudinal Zeeman sensitivities of 0.25 Mx/cm2 (Fe I 630.2 nm) and 0.5 Mx/cm2 (Ca II 854.2 nm). ViSP was operated in a "low" resolution mode (0.214" slit width, spectral resolution R ~ 70,000) to produce polarization maps over a common area of 105" x 50". Data from SDO and IRIS are combined to ask: Why is only a fraction of emerging flux filled with heated plasma? What is the elemental nature of the plasmas? No correlations were found between heated plasma and properties of chromospheric magnetic fields derived from the WFA, on scales below supergranules. Processes hidden from our observations control plasma heating. While improved magnetic measurements are needed, these data indicate that "the corona is a self-regulating forced system" (Einaudi et al. 2021). Heating depends on the state of the corona, not simply on boundary conditions. Heating models based upon identifiable bipolar fields, including cool loops, tectonics and observable magnetic reconnection, are refuted for these regions with unipolar chromospheric magnetic fields.

==> extras.tex <==

The striking 
difference between the relatively homogeneous 
network magnetic 
fields, Poynting flux proxies,  and the 
bright EUV emission 
has potentially 
pivotal consequence.  
The proxies derived from ViSP data clearly 
do not correlate with almost any of the overlying 
coronal emission. 
\subsection{no}


The magnetic field threading plasmas observed at UV and EUV wavelengths over the 
network boundaries are far more 
uniform in the mid-chromosphere than
in the photosphere, a property  often 
assumed and found in models 
\citep[e.g.][]{Gabriel1976,Carlsson+others2016},
while at the same time the thermal
structure is far more dynamic and intermittent. The very different 
emissions from plasmas threaded by 
the upward extension of these 
magnetic fields from spectra 
\ion{C}{2} to \ion{Fe}{9}
and \ion{Fe}{10} 
(Figures
\ref{fig:focus}
and \ref{fig:focuso}) demand 
a careful interpretation.

Such well-studied plasmas have undergone sophisticated analysis without taking into consideration 
the basic information uncovered here 
on these small
scales. This is striking 
because 
IRIS has observed 
transition region lines with 0.165$\arcsec$ pixels since June 2013, and as reported
in many publications
\citep[see the reviews of][]{Carlsson+others2019,dePontieu+others2022} they have been compared with ``advanced'' calculations.   Thus the question arises, would these
calculations be able to account for the lack of correlations seen in 
the images presented here?  If not, what do the differences imply? 




The data we have presented suggest that ordered energy
somehow leads to four different manifestations of
heated plasma:
\begin{itemize}
    \item the small bright blobs seen in the 
    IRIS \ion{C}{2} and \ion{Si}{4} slitjaw images, 
    \item quite different ``blobs'' of plasma generating \ion{He}{2} emission in AIA 30.4 nm images, 
    \item dimmer ``fibril'' emission extending as part of the chromospheric canopy
    expanding away from more intense network magnetic fields, and
    \item entirely independent 
    emission from genuinely coronal plasma ($T_e > 10^6$ K) only intermittently in space.
\end{itemize}
Each and every one of these 
observations must be explained in terms of magnetic fields which are demonstrably locally
unipolar on observable scales.
In a prescient paper, 
\citet{Litwin+Rosner1993}
inferred from spatially
intermittent coronal plasma implies
that heating \textit{to coronal temperatures} occurs
only when a certain threshold is reached.   Below this threshold, we can, as others have done before, 
speculate that radiation losses
deny the plasma the chance
of reaching coronal temperatures, even if it 
is heated to just below this threshold.  The observed variations in
time of coronal emission and the emissions from 
\ion{C}{2}, \ion{Si}{4}, and  \ion{He}{2} spectra are not inconsistent with 
radiation loss and dynamical
times for plasmas frozen into the extended, smooth chromospheric magnetic structure that pervades the upper atmosphere.   There are
many mechanisms capable of
dumping heat intermittently
along locally unipolar field
lines without large-scale 
reconnection, including 
the formation and decay of current sheets, resonant absorption or phase mixing of
intermediate MHD waves, as reviewed
in depth by \citet{Judge+Ionson2023}.  








 A common argument 
is that there is a lot of mixed polarity flux all over the Sun outside of strong spots, and that there is the  problem of Zeeman signal cancellation. Indeed,
for decades it has been recognized that
there is another component of magnetic field
which is, in terms of magnetic energy,
invisible to the Zeeman effect.
Using the Hanle effect which 
modifies atomic polarization induced by anisotropic processes, and measures field strength and not flux per unit area, fields of perhaps 10-80 Gauss 
have been inferred over large areas of quiet Sun \citep[e.g.][]{Kleint+Gandorfer2017}.  These are called
``turbulent'' fields precisely because they must lie below scales measured 
below resolution elements for them to
be invisible to the Zeeman effect. 
By itself this is sufficient to 
reject such fields as candidates for
cool loops. 

If we had merely measured photospheric magnetic fields, this argument might appeal to those
invoking a role for these fields
in energizing the solar transition region
and corona.  However, on scales of $150$ km, 
such ``salt and pepper'' fields clearly seen
in magnetograms (Figures~\ref{fig:focus} and
\ref{fig:focuso}), are absent in
the chromospheric accompanying magnetograms.
the inference is that these fields 
have not reached chromospheric heights
within these bright network flux concentrations.
This is as expected from considerations 
that the chromospheric fields exceed 
those measured using the Hanle effect. 

The behavior observed suggests that the transfer of ordered 
energy to plasma heating 
must occur
on unresolved scales, but which 
leads to 

from perhaps 100 km
where differential compressive motions can be converted to 
heat by ion viscosity, 
to the ion skin depth of 10 m.


 But perhaps the most important conclusion
we might draw is that \textit{the corona
exists above regions for long periods
with no clear physical connection to
the footpoints}, as evaluated using 
chromospheric magnetic properties.
This new
result is in addition to suggestive 
results obtained from the apparent  morphology of UV and EUV spectral images known for
some time \citep[e.g.][]{Berger+others1999}. 
         
Figure~\ref{fig:sens} is for the 
line-of-sight magnetic field
measurement data (not raw intensities).
\ion{Ca}{2} 854.2 line.  



A sobering corollary follows.  
When limited to measurements
of brightness alone,
(intensity), the fine structure distracts from
the fact that the magnetic field is dominant and so far less structured.  
\pja{The conclusion must be that in studying 
intensity images and spectra  of chromosphere, transition region and corona alone  (e.g.,
\citealp{Carlsson+others2019,dePontieu+others2021}), one is merely seeing the effects of magnetic free
energy, after 
plasma heating has already occurred
\citep{Judge+Ionson2023}.}



This
observation must relate to the failure of standard emission measure
analysis to account for Na-like and helium lines
\citep{Jordan1975,Jordan1980a,Pietarila+Judge2004,Judge+Pietarila2004}.


To illustrate this, we might assume that DKIST has
measured all \textit{chromospheric} magnetic fields on scales above
0.214 Mm. The data would then, \textit{under this assumption}, be conclusive: the bright cool loops can
connect\rc{\sout{ion}} the 2.2\% of pixels of opposite sign to regions of the
dominant polarity flux, producing an unobserved ``halo'' of bright TR
emission around the edges of the unipolar region.  This is contrary to
the data shown.




It seems that although the intensity of the magnetic field is
correlated to heating only on the largest scales
\citep[e.g.,][]{Fisher+others1998}, below a scale of few Mm, there is
no significant correlation.  This is consistent with Sturrock's
conjecture.  On smaller scales, bright plasmas become spatially
de-correlated (Table~\ref{tab:spearman}).
Observations of the Zeeman effect are unable to reveal
physical scales on which higher derivatives \rc{\textbf{\emph{(I presume you are referring to spatial derivatives... You should clarify the point you're making. I don't see why, apart from the known limitations of the Zeeman diagnostic (such as signal cancellation in the presence of a random field), one shouldn't be able to detect B variations across the FOV. If you're thinking along the LOS, I agree things become more difficult, but this is true for any type of magnetic diagnostic.)}}} of the magnetic field
might exist. Yet it is clear from magneto-hydrodynamics that sources
in the fluid energy equation vary as the square of the first spatial
derivatives of the magnetic and velocity vector fields, even if using
classical expressions for resistivity and viscosity respectively
\citep{Spitzer1956, Braginskii1965}. These classical coefficients
apply to plasmas in which deviations of all particles from Boltzmann
distributions are small. It remains questionable whether these may be
applied, as they are in all modern MHD ``advanced'' codes capable of
modeling coronal plasma \citep{Gudiksen+others2011,Rempel2017}. A
variety of dynamical instabilities may develop, before classical
physical transport occurs \citep{Judge+Ionson2023}.  No matter the
nature of this kind of unresolved dynamics which ultimately converts
ordered magnetic or kinetic energy into heat, the data analyzed here
support the notion that the zeroth derivatives of the emerging field,
the measurable magnetic field, 
have little to do with heating plasmas, except to define the
large-scale topology and Alfv\'en speeds.  This conclusion
might prompt re-examination of many earlier
MHD numerical experiments \citep[e.g.,][]{Einaudi+others2021,Howson+others2020} in which
the self-organizing nature of coronal plasma and heating
has been identified. 
We infer that there are727
processes outside of our current ability to measure, which728
must determine the rate of coronal heating.


Identifiable  
plasma loops exist for times $\tau$ 
far longer than the 
thermal cooling time $t$
(\citealp{Bray+Loughhead+Durrant1984,Judge 2023}), implying that the average dissipation rate $b^2/8\pi\tau$ needed for heating 
 the energy associated with the large scale magnetic field $\vec{B}_0$
defining the time-averaged topology.


The other proxy of Poynting flux 
conveniently highlights
the physics behind 
equation~(\ref{eq:decomp}) since 
$\frac{1}{2} \rho
\xi^2 c_A = \frac{1}{8\pi} b^2 c_A$. 


Correlations 
between the $B_{LOS}$ 630 data and the intensities of 
160 and 170 nm from AIA are larger than those between
$B_{LOS}$ 854 and the AIA data in Table~\ref{tab:spearman}.  


